$k$-SUM in the Sparse Regime

In the average-case $k$-SUM problem, given $r$ integers chosen uniformly at random from $\{0,\dots,M-1\}$, the objective is to find a ``solution'' set of $k$ numbers that sum to $0$ modulo $M$. In the dense regime of $M \leq r^k$, where solutions exist with high probability, the complexity of these problems is well understood. Much less is known in the sparse regime of $M\gg r^k$, where solutions are unlikely to exist. In this work, we initiate the study of the sparse regime for $k$-SUM and its variant $k$-XOR, especially their planted versions, where a random solution is planted in a randomly generated instance and has to be recovered. We provide evidence for the hardness of these problems and suggest new applications to cryptography. Complexity. First we study the complexity of these problems in the sparse regime and show: - Conditional Lower Bounds. Assuming established conjectures about the hardness of average-case (non-planted) $k$-SUM/$k$-XOR when $M = r^k$, we provide non-trivial lower bounds on the running time of algorithms for planted $k$-SUM when $r^k\leq M\leq r^{2k}$. - Hardness Amplification. We show that for any $M \geq r^k$, if an algorithm running in time $T$ solves planted $k$-SUM/$k$-XOR with success probability $\Omega(1/\text{polylog}(r))$, then there is an algorithm running in time $\tilde{O}(T)$ that solves it with probability $(1-o(1))$. - New Reductions and Algorithms. We provide reductions for $k$-SUM/$k$-XOR from search to decision, as well as worst-case and average-case reductions to the Subset Sum problem from $k$-SUM, as well as a new algorithm for average-case $k$-XOR at low densities. Cryptography. We show that by additionally assuming mild hardness of $k$-XOR, we can construct Public Key Encryption (PKE) from a weaker variant of the Learning Parity with Noise (LPN) problem than was known before.

==> equiv-alt-proof.tex <==
\section{Stronger Equivalence of Planted and Non-Planted $k$-SUM}\label{appendix:same_algorithm}

In this section, we present a proof of a stronger version of \cref{thm:planted_nonplanted_equivalence}, namely that the \emph{same} algorithm that solves the planted problem also solves the non-planted problem. Our main result is the following.

\begin{theorem}\label{thm:planted_nonplanted_equivalence_2}
    For any $k\in\Nat$ and ensemble $\G$ of density $1$, suppose there exists an algorithm that runs in time $T(r)$ and solves \emph{planted} search $k$-SUM over $\G$ with success probability at least $\epsilon(r)$. Then, the same algorithm also solves \emph{non-planted} search $k$-SUM over $\G$ with success probability at least $\epsilon(r)^{3/2}/6$.
\end{theorem}

At a high-level, we wish to show that any algorithm $\A$ that solves the planted $k$-SUM recovery problem with some constant probability $\epsilon>0$ also solves the non-planted $k$-SUM recovery problem with constant probability $\epsilon'>0$ for a possibly different constant. To do so, we proceed using a hybrid argument where we define a intermediate distribution, parameterized by some integer $\ell > 0$, whose distance to both $D_0$ and $D_1$ can be bounded. By transitivity, this shows that $D_0$ and $D_1$ are also close and allows us to bound the error probability. In the former case, we are able to bound the Rényi divergence, and in the latter the statistical distance. This allows us to express $\epsilon'$ as an affine function of $\epsilon$, i.e. $\epsilon' = \alpha \epsilon - \beta$ where $\alpha=\alpha(\ell)$ and $\beta=\beta(\ell)$ are functions of $\ell$. We will show that, for each $\epsilon$, there is a choice of $\ell$ such that $\epsilon' > 0$ for sufficiently large $r$, which would conclude the proof.


Specifically, we define the following family of probability distributions, 
\paragraph{Distribution $D^{\ell}$}
\begin{enumerate}
    \item Sample $X \sample D_1$.
    \item Let $c(X)$ be the number of solutions.
    \item If $c(X) > \ell$, let $X \sample D_0$.
    \item Output $X$.
\end{enumerate}
Note that this distribution `interpolates' between $D_0$ and $D_1$ - in particular, we have $D^{0} = D_0$ and $D^{\binom{r}{k}} = D_1$.

\begin{lemma}\label{lemma:explicit_pmf}
  For any $X$, if $c(X)$ is the number of solutions in $X$, we have,
    \begin{enumerate}
        \item $D_1(X) = c(X) \,D_0(X)$.
        \item $D^\ell(X) = \left(\one[c(X) \leq \ell]\,c(X) + \underset{X \sim D_1}{\Pr}[c(X) > \ell]\right) D_0(X)$.
    \end{enumerate}
\end{lemma}
\begin{proof}
    The first statement is just \cref{lemma:explicit_pmf just D_1}. To prove the second statement, observe that $D^\ell(X)$ is the sum of the probability of choosing $X$ in step 1 and that of choosing $X$ in step 3 of the sampling procedure. The first term is clearly 0 if $c(X)>\ell$ (since step 3 would override it in that case) and $D_1(X)$ otherwise. The second term is the product of the probability of re-sampling in step 3 (which is exactly $\underset{X\sim D_1}{\Pr}[c(X)>\ell]$) and the probability of getting $X$ from re-sampling (which is just $D_0(X)$). The statement now follows from adding the two terms and expanding $D_1(X)=c(X)D_0(X)$.
\end{proof}

Next, we will bound the Rényi divergence of $D^\ell$ and $D_0$ using \cref{lemma:renyi} which gives a multiplicative bound on the error. In fact, applying \cref{lemma:explicit_pmf}, it is straight-forward to bound the Rényi divergence for our use-case.
\begin{corollary}\label{cor:renyi}
    $R(D^\ell \lVert D_0) = \ell + \underset{X \sim D_1}{\Pr}[c(X) > \ell]$.
\end{corollary}
This establishes that $D^\ell$ is not `too far' from $D_0$ and establishes a multiplicative bound on the error probabilities for an algorithm that solves the hybrid distribution, and the non-planted distribution. Next, we will bound the statistical distance between $D^\ell$ and $D_1$ to get an additive bound.

\begin{lemma}\label{lemma:sd}
    $SD(D^\ell, D_1) < \frac{1}{(\ell-2)^2}$.
\end{lemma}
\begin{proof}
    At a high level, our proof strategy is to bound the statistical distance in terms of the probability that a planted instance has at least a certain number of solutions that we can then bound using Chebyshev's inequality by bounding its first two moments. 
    \begin{align*}
        SD&(D^\ell, D_1) \\
        &= \frac12 \sum_{X \in G^r} \left\lvert D^\ell(X) - D_1(X) \right\rvert\\
        &= \frac12 \left(\sum_{\underset{c(X) \leq \ell}{X \in G^r}} \underset{X \sim D_1}{\Pr}[c(X) > \ell]\, D_0(X)  + \sum_{\underset{c(X) > \ell}{X \in G^r}} \left[c(X) - \underset{X \sim D_1}{\Pr}[c(X) > \ell]\right] D_0(X) \right)\\
        &= \sum_{\underset{c(X) \leq \ell}{X \in G^r}} \underset{X \sim D_1}{\Pr}[c(X) > \ell]\, D_0(X)\text{\pnote{Should explain this equality} \nnote{identify X for which Dl(X) >= D1(X). This is exactly the probability of c(X)<=l. Hence, the SD is just the difference between Dl and D1 (which is this)}}\\
        &= \underset{X \sim D_1}{\Pr}[c(X) > \ell] \frac{\left\lvert \{X \in G^r \mid c(X) \leq \ell\} \right\rvert}{2^{mr}}\\
        &= \underset{X \sim D_1}{\Pr}[c(X) > \ell] \cdot \underset{X \sim D_0}{\Pr}[c(X) \leq \ell]\\
        &\leq \underset{X \sim D_1}{\Pr}[c(X) > \ell]
    \end{align*}
    Now, suppose we sample $X$ from $D_1$ and consider the number of solutions in $X$. Clearly, the number of solutions is invariant to where exactly the solution is planted, so we may condition on the event that the planted solution is $[k]$.
    
    Let $X \sim D_1$, let $S \subseteq [r]$ be a $k$-set and let $I_S = \one[\sum_{i \in S} X_i = 0]$ be the random variable, indicating whether $S$ is a solution for the instance $X$. Clearly, as $X$ is sampled randomly, we have $I_S \sim \Ber_2^{-m}$; hence $\E[I_S] = 2^{-m}$, and $\Var(I_S) = 2^{-m}(1-2^{-m})$. Now, let $I = \sum_{\underset{|S|=k}{S \subseteq [r]}} I_S = c(X)$ be the total number of solutions. First, note that by linearity of expectation,
    \begin{align*}
        \E[I] 
        &= \sum_{\underset{|S|=k}{S \subseteq [r]}} \E[I_S]
         = 1 + \sum_{\underset{|S|=k,\,S\neq [k]}{S \subseteq [r]}} 2^{-m}
         = 1 + \left({\binom{r}{k}} - 1\right)\, 2^{-m} = 2 - 2^{-m}
    \end{align*}
    Next, we may decompose the variance of $I$ as follows.
    \begin{align*}
        \Var(I) 
        &= \sum_{\underset{|S|=k}{S \subseteq [r]}} \Var(I_S) + \sum_{\underset{|S|=k}{S \subseteq [r]}} \sum_{\underset{\underset{T \neq S}{|T|=k}}{T \subseteq [r]}} \Cov(I_S, I_T)
    \end{align*}
    We shall make use of the fact that for the vast majority of tuples, the covariance is zero. In fact, we note the following identity.
    $$
        \Cov(I_S, I_T) = 
        \begin{cases}
            0 & \text{if $S \Delta T \neq [k]$}\\
            2^{-m}\,(1-2^{-m}) & \text{if $S \Delta T = [k]$}
        \end{cases}
    $$
    To see why this is true, note that when $S \Delta T = [k]$, since we know $[k]$ is a solution, we have that $I_S = I_T$ and hence $\Cov(I_S,I_T) = \Var(I_S) = 2^{-m}\,(1-2^{-m})$. On the other hand, if this is not the case, then $S$ must contain at least one group element contained in neither $T$ nor $[k]$, and hence $S$ is a solution for exactly one choice of this element, meaning $I_S$ is independent of $I_T$. This allows us to write,
    \begin{align*}
        \Var(I) 
        &= 1-2^{-m} + {\binom{k}{k/2}} {\binom{r-k}{k/2}}\,2^{-m}\,(1-2^{-m})\\
        &\leq 1-2^{-m} + c_k {\binom{r}{k-1}}\,2^{-m}\,(1-2^{-m})\\
        &\leq 1-2^{-m} + c_k \frac1r {\binom{r}{k}}\,2^{-m}\,(1-2^{-m})\\
        &= 1-2^{-m} + \frac{c_k (1-2^{-m})}{r}
    \end{align*}
    Here $c_k$ is a constant that depends only on $k$. Suppose for simplicity that $\Var(I) \leq 1$\pnote{Better to not say this and carry over the $o(1)$, as it will show up in the final bound}\nnote{This is not exactly true; add $o(1)$ and propagate it along}. We now put things together.
    \begin{align*}
        SD(D^\ell, D_1)
        &\leq \underset{X \sim D_1}{\Pr}[c(X) > \ell]\\
        &\leq \underset{X \sim D_1}{\Pr}[\left\lvert c(X) - 2\right\rvert > \ell - 2]\\
        &= \underset{X \sim D_1}{\Pr}[\left\lvert I - \E[I]\right\rvert > (\ell - 2)\Var(I)]\text{\pnote{Should be standard deviation to apply Chebyshev}}\\
        &\leq \frac{1}{(\ell-2)^2}
    \end{align*}
    Where the latter inequality follows from application of Chebyshev's inequality (\cref{lemma:chebyshev}).
\end{proof}

This establishes that $D^\ell$ is not `too far' from $D_1$, and implies a bound on the additive error between the success of an algorithm for the planted distribution and its success on $D^\ell$. 
\begin{figure}
    \centering
    \begin{tikzpicture}
        \node (D0) at (0,0) {$D_0$};
        \node (D1) at (12,0) {$D_1$};
        \node (Dl) at (6,-2) {$D^{(\ell)}$};
        \draw[dashed,color=gray] (D0) -- (D1);
        \draw (D0) to[bend right=15] node[fill=white]{Rényi divergence} (Dl);
        \draw (Dl) to[bend right=15] node[fill=white]{Statistical distance} (D1);
    \end{tikzpicture}
    \caption{Depiction of the argument for statistical closeness of $D_0$ and $D_1$. We define a class of hybrid distributions $D^{(\ell)}$ for which we can bound the distance to $D_0$ and $D_1$, specifically we bound the Rényi divergence between $D_0$ and $D^{(\ell)}$ and the statistical distance between $D^{(\ell)}$ and $D_1$. We show that for large enough values of $r$, there is an $\ell$ such that the nonplanted error probability on of any algorithm that solves the planted problem is some constant $>0$.}
\end{figure}

\paragraph{Proof of \cref{thm:planted_nonplanted_equivalence_2}.} We now prove the main result of this section. Let $\A$ be an algorithm that solves planted $k$-SUM, and let $\epsilon>0$ be a constant that lower bounds its error probability. We shall prove that $\A$ solves non-planted $k$-SUM with probability $\geq \epsilon'$ for some other constant $\epsilon'>0$. By \cref{lemma:sd,cor:renyi}, we get that,\pnote{State the bound on $\underset{X \sim D_1}{\Pr}[c(X) > \ell]$ as a separate claim above so it can be invoked here}
$$
    \epsilon' \geq \frac{\epsilon - \underset{X \sim D_1}{\Pr}[c(X) > \ell]}{\ell + \underset{X \sim D_1}{\Pr}[c(X) > \ell]} \geq \frac{\epsilon - \frac{1}{(\ell-2)^2}}{\ell + \frac{1}{(\ell-2)^2}}
$$
To ensure that $\epsilon'>0$, solving for $\ell$, we get that $\ell > 2 + \frac{1}{\sqrt{\epsilon}}$. Note that for any $\epsilon$ and $k$, there is a viable $\ell$ for sufficiently large $r$, which concludes the proof. \pnote{Using $\ell=2+\frac{2}{\sqrt{\eps}}$ should give the parameters stated in the theorem statement.} $\hfill\qed$

\begin{proofof}{\cref{thm:stat_indist}}
    Let $M$ be the set of instances without a solution. By \cref{lemma:explicit_pmf just D_1}, we know that $D_1$ has the property that $D_1(X) = 0$ for every $X \in M$ and that $D_1(X) \geq D_0(X)$ for every $X \in \supp(D_1)$. Hence, we get that,
\begin{align*}
    \Delta\left(D_0, D_1\right) = \sum_{X \in M} D_0(X) = \frac{|M_r|}{2^{mr}} &= \underset{X \sim D_0}{\Pr}[c(X) = 0] = 1 - \underset{X \sim D_0}{\Pr}[c(X) \geq 1]
\end{align*}
Our goal is thus to lower bound the probability that $X$ has at least one solution. We proceed in a similar manner as for the proof of \cref{lemma:density 1 at least half prob of solution}. We note again that by linearity of expectation the expected number of solutions satisfies,
$$
    \underset{X \sim D_0}{\E}[c(X)] = \binom{r}{k}\, 2^{-m} = \binom{r}{k}^{1-\frac1\Delta}.
$$
Similarly, since the indicator variables for two separate solutions are pairwise independent, we get that,
$$
    \underset{X \sim D_0}{\Var}[c(X)] = \binom{r}{k}^{1-\frac1\Delta}\,(1-2^{-m}).
$$
And thus we get that by application of Paley-Zygmund (\cref{lemma:paley_zygmund}) that, \pnote{Have to be a little careful below, as in Paley-Zygmund, the inequality in the probability in the left-hand side is strict. Shouldn't matter for the final result, in fact, it would even be simpler to bound $\Pr[c(X)>0]$.}
\begin{align*}
    \underset{X \sim D_0}{\Pr}[c(X) \geq 1]
    = \underset{X \sim D_0}{\Pr}\left[c(X) \geq \binom{r}{k}^{\frac1\Delta-1} \E[c(X)]\right]
    &\geq \frac{\left(1- \binom{r}{k}^{\frac1\Delta-1}\right)^2\,\E[c(X)]^2}{\binom{r}{k}^{1-\frac1\Delta}+\left(1- \binom{r}{k}^{\frac1\Delta-1}\right)^2\,\E[c(X)]^2}\\
    &=1-\frac{\binom{r}{k}^{1-\frac1\Delta}}{1 + \binom{r}{k}^{1-\frac1\Delta}\left(\binom{r}{k}^{1-\frac1\Delta}-1\right)}\\
    &\geq 1 - \frac{2}{\binom{r}{k}^{1-\frac1\Delta}}.
\end{align*}
This means we can upper bound the statistical distance as follows.
\begin{align*}
    SD\left(D_0, D_1\right) 
    &\leq \frac{2}{\binom{r}{k}^{1-\frac1\Delta}} \leq \frac{2}{\left(\frac{r}k\right)^{k[1-\frac1\Delta]}} = O\left({r^{k\left[\frac1\Delta-1\right]}}\right). \qedhere
\end{align*}
\end{proofof}

==> lncs_issues.tex <==
%!TEX root = main.tex

%% Fixes to lncs class

\makeatletter
\def\@thmcountersep{.}
\def\@thmcounterend{.}

\def\spnewtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \spnewtheorem with number

\def\@spnthm#1#2{%
	\@ifnextchar[{\@spxnthm{#1}{#2}}{\@spynthm{#1}{#2}}}
\def\@Sthm#1{\@ifnextchar[{\@spothm{#1}}{\@spnthm{#1}}}

\def\@spxnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
	{\@definecounter{#1}\@addtoreset{#1}{#3}%
		\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
			\csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@spynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
	{\@definecounter{#1}%
		\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#3}{#4}}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@spothm#1[#2]#3#4#5{%
	\@ifundefined{c@#2}{\@latexerr{No theorem environment `#2' defined}\@eha}%
	{\expandafter\@ifdefinable\csname #1\endcsname
		{\newaliascnt{#1}{#2}%
			\expandafter\xdef\csname #1name\endcsname{#3}%
			\global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
			\global\@namedef{end#1}{\@endtheorem}}}}

\def\@spthm#1#2#3#4{\topsep 7\p@ \@plus2\p@ \@minus4\p@
	\refstepcounter{#1}%
	\@ifnextchar[{\@spythm{#1}{#2}{#3}{#4}}{\@spxthm{#1}{#2}{#3}{#4}}}

\def\@spxthm#1#2#3#4{\@spbegintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
	\ignorespaces}

\def\@spythm#1#2#3#4[#5]{\@spopargbegintheorem{#2}{\csname
		the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\@spbegintheorem#1#2#3#4{\trivlist
	\item[\hskip\labelsep{#3#1\ #2\@thmcounterend}]#4}

\def\@spopargbegintheorem#1#2#3#4#5{\trivlist
	\item[\hskip\labelsep{#4#1\ #2}]{#4(#3)\@thmcounterend\ }#5}

% definition of \spnewtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
	{\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
		\expandafter\xdef\csname #1name\endcsname{#2}%
		\global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\topsep 7\p@ \@plus2\p@ \@minus4\p@
	\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
	{#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
	\item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
	\item[\hskip\labelsep{#3#1}]{#3(#2)\@thmcounterend\ }}

%\if@envcntsect
%\def\@thmcountersep{.}
%\spnewtheorem{theorem}{Theorem}[section]{\bfseries}{\itshape}
%\else
%\spnewtheorem{theorem}{Theorem}{\bfseries}{\itshape}
%\if@envcntreset
%\@addtoreset{theorem}{section}
%\else
%\@addtoreset{theorem}{chapter}
%\fi
%\fi

%definition of divers theorem environments
\if@envcntsame % alle Umgebungen wie Theorem.
\def\spn@wtheorem#1#2#3#4{\@spothm{#1}[theorem]{#2}{#3}{#4}}
\else % alle Umgebungen mit eigenem Zaehler
\if@envcntsect % mit section numeriert
\def\spn@wtheorem#1#2#3#4{\@spxnthm{#1}{#2}[section]{#3}{#4}}
\else % nicht mit section numeriert
\if@envcntreset
\def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
	\@addtoreset{#1}{section}}
\else
\def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
	\@addtoreset{#1}{chapter}}%
\fi
\fi
\fi


\spn@wtheorem{fact}{Fact}{\bfseries}{\itshape}
\spn@wtheorem{assumption}{Assumption}{\bfseries}{\itshape}
\spn@wtheorem{myclaim}{Claim}{\bfseries}{\itshape}
\Crefname{myclaim}{Claim}{Claims}
\makeatother

==> pke_2.tex <==
\section{Full Public-Key Encryption from $2^{m^{0.5}}$-hardness of Constant-Noise LPN}\label{appendix:pke2}
In this appendix, we provide a construction of (strong) PKE based on $2^{m^{0.5}}$-hardness of LPN with constant noise. We will essentially be repeating the construction from \cref{sec:pke} and repeat it independently $\ell$ number of times. We show that the cryptosystem satisfies the following definition (adapted from \cite{pke_amplification}).

\begin{definition}[Public-Key Encryption]
    Let $PKE=\langle \KeyGen_\lambda, \Enc_\lambda, \Dec_\lambda \rangle$ be a triple of function families, parameterized by a security parameter $\lambda \in \mathbb{N}$. We say $PKE$ is an \emph{$(\varepsilon, \delta)$-secure public key bit encryption scheme} if it satisfies the following two properties.
    \begin{itemize}
      \item \emph{($\varepsilon$-Correctness).} For any $\lambda \in \mathbb{N}$,
        $$
            \Pr\left[\Dec_\lambda(sk, \Enc_\lambda(pk, b)) = b \right] \geq 1-\varepsilon(\lambda),
        $$
        whenever $\langle pk, sk \rangle \gets \KeyGen_\lambda()$, where the randomness is taken over $b$ and the random coins used by $PKE$.
        \item \emph{($\delta$-Indistinguishability).} For any PPT adversary $\A$, it holds that,
        $$
            \Pr\left[\A(pk, \Enc_\lambda(pk, b)) = b\right] \leq \frac{1 + \delta(\lambda)}2,
        $$
        whenever $\langle pk, sk \rangle \gets \KeyGen_\lambda()$, where the randomness is taken over $b$ and the random coins used by $PKE$.
    \end{itemize}
    If both $\varepsilon, \delta$ are negligible functions in the security parameter, we say $PKE$ is a \emph{secure public-key bit encryption scheme}.
\end{definition}

We now describe formally the cryptosystem where the security parameter is the number of vectors $\lambda$ to generate in the public key. The cryptosystem is denoted $PKE_{k,\ell,m}$ and is parameterized by three functions $k,\ell,m : \Nat \rightarrow \Nat$ where
$$
    \Delta_k^{(\lambda)} = \frac{k(\lambda) \log \lambda}{m(\lambda)}
$$ 
determines the density of the generated instances, and $\ell(\lambda)$ determines the number of independent repetitions of the simple cryptosystem described in the introduction. We will use $k,\ell,m$ in lieu of $k(\lambda),\ell(\lambda),m(\lambda)$ when $\lambda$ is clear from the context.

\paragraph{Key Generation $\KeyGen_\lambda$.}
\begin{enumerate}
    \item  Let $pk \sample \F_2^{m(\lambda) \times \lambda}$.
    \item Choose a random set $sk \subseteq [\lambda]$ with $|sk|=k(\lambda)$.
    \item Let $i \in sk$ be the smallest index and let $pk_{i} \gets - \displaystyle\sum_{\underset{j \neq i}{j \in sk}} pk_{j}$.
    \item Return $\langle pk, sk \rangle$.
\end{enumerate}

\noindent Here, we will interpret each $sk \in \F_2^\lambda$ as the characteristic vector for the set $sk \subseteq [\lambda]$.

\paragraph{Encryption $\Enc_\lambda(pk, b)$.}
\begin{enumerate}
    \item If $b=0$.
    \begin{enumerate}
        \item[1.1.] Return $C \sample \F_2^{\ell(\lambda) \times \lambda}$.
    \end{enumerate}
    \item If $b=1$.
    \begin{enumerate}
        \item[2.1.] Let $S \sample \F_2^{\ell(\lambda) \times m(\lambda)}$.
        \item[2.2.] Let $E \gets \Ber_{\eta/2}^{\ell(\lambda) \times \lambda}$.
        \item[2.3.] Return $C \gets S\, pk + E$.
     \end{enumerate}
\end{enumerate}

\paragraph{Decryption $\Dec_\lambda(sk, C)$.}
\begin{enumerate}
  \item Return $0$ if $\lVert C \, sk \rVert_0 > \ell \left(\frac12 + \frac{{(1-\eta)}^{k}}{4}\right)$; else return 1.
\end{enumerate}

\begin{lemma}\label{lemma:epsilon-correctness}
    The cryptosystem is $\varepsilon$-correct when $\ell \geq 32 \left(1-\eta\right)^{2 k}\ln(1/\varepsilon)$.
\end{lemma}
\begin{proof}
    Suppose for $\ell=1$ that we encrypt $b=0$ such that $c$ is a uniformly random vector from $\{0,1\}^r$. It is clear in this case, as $sk \neq 0^r$, that $sk^\top c_i$ a uniformly random bit, i.e. if $\langle pk, sk \rangle \gets \KeyGen(r)$, then we get that, $
        \Pr[\Dec(\Enc(0, pk), sk) = 1] = \frac12$. If instead we encrypt $b=1$ and there are no errors in the $k$ positions corresponding to the planted set, then decryption will be correct. This happens with probability $(1-\eta)^k$. If instead, some error occurred in the planted set, decryption will be correct with probability $\frac12$. As such, 
        $$
            \Pr[\Dec(\Enc(1,pk),sk)=1] = (1-\eta)^{k} +  \frac{1-(1-\eta)^k}2.
        $$
        This does not provide useful correctness by itself so we amplify the difference by repeating the process $\ell$ and taking majority vote. Now suppose we have $\ell$ iterations and consider the case of $b=0$. Let $E_i = c_i^\top sk$, for $i=1\ldots \ell$. Then all $E_i$ are i.id. and satisfy $\E[E_i] = \frac12$. It follows by a Chernoff bound (\cref{lemma:chernoff}) that,
    \begin{align*}
        \Pr[\Dec(\Enc(0,pk),sk)=1] 
        &= \Pr\left[\sum_{i=1}^\ell E_i \leq \ell \left(\frac12 + \frac{(1-\eta)^{k}}{4}\right)\right]
        \leq e^{-\left(\frac14\left(1-\eta\right)^{k}\right)^2 \ell / 2}.
    \end{align*}
    This gives a decryption error of at most $\varepsilon$ whenever $\ell \geq 32 \left(1-\eta\right)^{2 k}\ln(1/\varepsilon)$. The case for $b=1$ is identical.
\end{proof}

Unlike many cryptographic assumptions, the search and decision LPN problems are known to be polynomially equivalent, as showed in \cite{lpn_search_decision}. We restate their result as follows.
\begin{lemma}[Katz, Shin, Smith, \cite{lpn_search_decision}]\label{lemma:lpn search decision equiv}
    If there is an algorithm that runs in time $T$ and solves the decision LPN problem with advantage $\epsilon$, then there is an algorithm that runs in time $\mathcal{O}\left(\frac{T\,m \log m}{\epsilon^2}\right)$ and solves the search LPN problem with probability $\epsilon/4$.
\end{lemma}

To prove security of our public-key encryption scheme, we will put forth the following assumption.
\begin{assumption}[Sub-exponential Hardness of Constant-Noise LPN]\label{ass:lpn}
There is a constant $c>0$, such that for $\eta=\Theta(1)$, then any algorithm that runs in time $2^{\mathcal{O}\left(m^c\right)}$ has advantage $o(1)$ in the search LPN problem over $\F_2$ with noise rate $\eta$.
\end{assumption}
This assumption for $c=0.5$ was already known to be sufficient to construct collision-resistant hashing \cite{lpn_crh} as well as public-key encryption \cite{lpn_pke}. We present our construction mainly for completeness, though it is arguably also qualitatively simpler than the one presented in \cite{lpn_pke}. 

We can leverage the equivalence of \cref{lemma:lpn search decision equiv} to to translate \cref{ass:lpn} into a stronger bound on the advantage of an algorithm that solves decision LPN. Consider 
\begin{corollary}\label{cor:lpn_decision_adv}
    Under \cref{ass:lpn}, there is no algorithm  that runs in time $2^{\mathcal{O}\left(m^c\right)}$ and solves the decision LPN problem for $\eta$ with advantage $> \frac{1}{2^{\Omega\left(m^c\right)}}$.
\end{corollary}


\begin{theorem}\label{theorem:pke}
    Using $k$-XOR at constant density, there are $k,\ell,m$ such that $PKE_{k,\ell,m}$ is a secure public-key bit encryption scheme if only if \cref{ass:lpn} holds for some $c \geq \frac12$.
\end{theorem}
\begin{proof}
The idea is to work in a constant density slightly larger than 1 (say $\epsilon$) and use a superconstant $k$. We then leverage the statistical closeness of \cref{lemma:sd} to conclude that the $k$-XOR detection problem is hard. We then hope to be able to instantiate $m$ such that LPN is also hard. Suppose we define the following parameters. 
\begin{align*}
    \eta = \Theta(1) &&
    k = \epsilon\,(\log \lambda)^\alpha &&
    m = (\log \lambda)^\beta &&
    \ell = \Theta((\log \lambda)^2)
\end{align*}
Here, we need $\alpha > 0$ for $k$ to be superconstant. The constraint $\ell = \textsf{exp}(k)\, \omega(\log \lambda)$ is needed by \cref{lemma:epsilon-correctness} to ensure we have negligible decryption error; so we may let $\ell = \Theta((\log \lambda)^2)$. Note that in order for the ciphertext to be polynomial, this requires us to have $0 < \alpha \leq 1$. Also note that the density in our case is $\epsilon \frac{k \log r}{m} = (\log \lambda)^{\alpha + 1 - \beta}$ which means we need $\beta = \alpha+1$ to obtain constant density.

For indistinguishability, we proceed using a hybrid argument and define the distribution $H_b^{(i)}$ that generates a public key $pk$ using the distribution $D_b$, generates $i$ vectors of the form $s^\top pk + e^\top$ and $\ell-i$ random vectors from $\F_2^\lambda$. Note that $H_1^{(0)}$ is an encryption of 0 and $H_1^{(1)}$ is an encryption of 1. By \cref{cor:lpn_decision_adv}, we can bound the advantage by,
\begin{align*}
    \frac{(\log \lambda)^2}{2^{m^c}} = \frac{(\log \lambda)^2)}{2^{(\log \lambda)^{\beta c}}},
\end{align*}
which is negligible when $c > \frac{1}{\beta} = \frac1{\alpha + 1}$ which -- as $\alpha \in (0,1]$ -- implies that $c \geq \frac12$ as needed.
\end{proof}

\begin{figure}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tikzpicture}
        \node at (0,1) {$(pk, \Enc(pk,0))$};
        
        \draw[dashed,color=gray] (0.5,0) -- (14.5,0);
        
        \draw (-0.5,-0.5) rectangle (0.5,0.5);
        \node at (0,0) {$H_1^{(0)}$};

        \draw (0,-0.5) -- (0,-2.5);

        \draw (-0.5,-2.5) rectangle (0.5,-3.5);
        \node at (0,-3) {$H_0^{(0)}$};
        
        \draw (0.5,-3) -- (4.5,-3);
        
        \draw (4.5,-2.5) rectangle (5.5,-3.5);
        \node at (5,-3) {$H_0^{(1)}$};
        
        \draw (5.5,-3) -- (14.5,-3);
        
        \node[fill=white] at (10,-3) {$\cdots$};
        
        \draw (14.5,-2.5) rectangle (15.5,-3.5);
        \node at (15,-3) {$H_0^{(\ell)}$};

        \draw (15,-0.5) -- (15,-2.5);
        
        \node at (15,1) {$(pk, \Enc(pk,1))$};
        \draw (14.5,-0.5) rectangle (15.5,0.5);
        \node at (15,0) {$H_1^{(\ell)}$};
        
        \node[fill=white] at (0,-1.3) {(\cref{thm:stat_indist})};
        \node[fill=white] at (0,-1.7) {$\approx$};
        
        \node[fill=white] at (15,-1.3) {(\cref{thm:stat_indist})};
        \node[fill=white] at (15,-1.7) {$\approx$};
        
        \node[fill=white] at (2.5,-2.8) {(\cref{ass:lpn})};
        \node[fill=white] at (2.5,-3.2) {$\approx$};
        
        \node[fill=white] at (7.5,-2.8) {(\cref{ass:lpn})};
        \node[fill=white] at (7.5,-3.2) {$\approx$};
        
        \node[fill=white] at (12.5,-2.8) {(\cref{ass:lpn})};
        \node[fill=white] at (12.5,-3.2) {$\approx$};
    \end{tikzpicture}
    }
    \caption{Structure of the hybrid argument. The distribution $H_b^{(i)}$ generates a public key $pk$ using the distribution $D_b$, generates $i$ vectors of the form $s^\top pk + e^\top$ and $\ell-i$ random vectors from $\F_2^r$. The distribution $H_1^{(0)}$ thus corresponds to an encryption of 0, while $H_1^{(\ell)}$ is an encryption of 1. By the $k$-XOR conjecture at density 1 for $k=(\log \log r)^2$ (\cref{ass:kxor_1}) and our recovery-to-detection reduction (\cref{thm:recovery_to_detection}), we have that $H_1^{(0)}$ (respectively, $H_1^{(\ell)}$) is $o(1)$-indistinguishable to $H_0^{(0)}$ (respectively, to $H_0^{(\ell)}$) where the public key is replaced by a random matrix. Similarly, the LPN conjecture implies that $H_0^{(i)}$ is $o(1)$-indistinguishable to $H_0^{(i+1)}$ for every $i \in [\ell]$. We conclude the argument by noting that $\ell$ is a constant.}
    \label{fig:my_label}
\end{figure}

==> pke_lwe.tex <==
\section{Public Key Encryption}
\label{sec:pke}

%\prashant{Can some exponential hardness of LWE with minicrypt-level noise give PKE on its own without needing $k$-SUM?}\shweta{Akhil and I have been discussing this and we think the answer is no, which is good for us.}



%\shweta{The hardness of LWE depends on the approximation factor $n/\alpha$ of the underlying gapsvp problem. Typically this is $1/poly$, for us, it can be constant. I think we can use LWE with constant $\alpha$ to construct SKE not PKE. Argue this. }
%\shweta{Any particular reason we chose dual Regev from GPV08 rather than primal Regev from Reg05?}\akhil{No, it was more of my personal choice, but using primal sort of avoids the need to use a targeted version. So, i changed it to primal.}

\subsection{Definitions}
\label{sec:pke-defs}

\begin{definition}[Public Key Encryption] \label{def:pke}
    A \emph{Public Key Encryption (PKE)} scheme for a message space $\cM$ consists of PPT algorithms $\pke = (\keygen, \enc, \dec)$ with the following syntax:

\begin{itemize}
    \item $\keygen(1^{\secp}) \xrightarrow{} (pk, sk)$: on input the unary representation of the security parameter $\secp$, generates a public key $pk$ and a secret key $sk$.
    \item $\enc(pk,m) \xrightarrow{} ct$: on input a public key $pk$ and a message $m \in \cM$, outputs a ciphertext $ct$.
    \item $\dec(sk,ct) \xrightarrow{} m$: on input a secret key $sk$ and a ciphertext $ct$, outputs a message $m \in \cM$.
\end{itemize}
The scheme should satisfy the following properties:
    \begin{description}
        \item \textbf{Correctness}. A scheme $\pke$ is \emph{correct} if there exists a negligible function $\negl$ such that for every security parameter $\secp$ and message $m \in \cM$ :
        \begin{equation*}
            \Pr[\dec(sk, \enc(pk, m)) = m] \geq 1 - \negl(\secp) %\akhil{\text{Replace negl with o(1) for weak correctness}}
        \end{equation*}
        where $(pk, sk) \gets \keygen(1^{\secp})$.
    The scheme is \emph{weakly} correct if the probability of correct decryption is bounded by $1 - o(1)$ instead of $1 - \negl(\secp)$ above.
        
     \item \textbf{CPA Security}. A scheme $\pke$ is \emph{IND-CPA secure} if for any PPT adversary $\sfA$ there exists a negligible function $\negl$ such that: 
        \begin{equation*}
        \label{eq:indcpa}
        \big|\Pr[\pkeGame_{\sfA(\secp)}^{0} = 1] - \Pr[\pkeGame_{\sfA(\secp)}^{1} = 1]\big| \leq  \negl(\secp)
        \end{equation*}
        where $\pkeGame_{\sfA(\secp)}^{b}$ is a game between an adversary $\sfA$ and a challenger $\sfC$ with a challenge bit $b$ defined as follows:
        \begin{itemize}
            \item $\sfC$ samples $(pk, sk) \gets \keygen(1^{\secp})$, and sends $pk$ to $\sfA$.
            \item $\sfA$ chooses $m_{0}, m_{1} \in \cM$ and sends them to $\cC$.
            \item $\sfC$ computes $ct \gets \enc(pk, m_{b})$, and sends $ct$ to $\sfA$.
            \item The adversary $\sfA$ outputs a bit $b'$ which we define as the output of the game.
        \end{itemize}
        The scheme is said to be \emph{weakly} IND-CPA secure if we replace $\negl(\secp)$ with $o(1)$ in the condition above. 
    \end{description}    
 \end{definition}  
\begin{definition}[The $\vkSUM$ problem]\label{def:vkSUM}
   Let $n$, $m = m(n)$, $k=k(n)$, and $q = q(n)$ be integers. The $\vkSUM(n,m,k,q)$ problem is to distinguish between the following distributions:
    \begin{itemize}
        \item $(\veca_1, \veca_2, \ldots, \veca_n)$, where each $\veca_i$ is chosen uniformly from $\Z_{q}^{m}$.
        \item $(\veca_1, \veca_2, \ldots, \veca_n)$, where each $\veca_i$ is chosen uniformly from $\Z_{q}^{m}$, and then for a uniformly chosen set $S\subset[n]$ of size $k$, we set $\veca_j = - \sum_{i \in S \setminus \{j\}} \veca_i$, where $j = \min_{i \in S} i$.
    \end{itemize}
\end{definition}

We prove the following lemma in \cref{sec:vector-ksum}.\prashant{Say how at low densities this can be solved by Gaussian elimination, just like $\kXOR$}

\begin{restatable}{lemma}{vectorksum}
\label{reduction-vkSUM}
    If there is  an algorithm that solves $\svkSUM(n,m,k,q)$ in time $T(n)$ with success probability $\eps$, then there is an algorithm that solves $\skSUM(n,k,q)$ in time $O(T(n)\cdot k^m)$ with success probability $\eps$.\prashant{Please check the values for the success probabilities. Currently this statement is for the search problems. Modify this and its proof to be for the decision versions instead.}
\end{restatable}

% The $\vkSUM(n,m,k,q)$ problem can also be conjectured hard for some regime of parameters. Specifically, we provide the following conjecture and justify it in Lemma \ref{reduction-vkSUM}.
% \begin{conjecture}\label{conj:vkSUM}
% For any $n, m=m(n), k=k(n), q = q(n),\Delta=\ceil{\frac{k\log{n}}{m\log{q}}}$, any adversary that runs in time $n^{\ceil{k/2}(1-\Omega(1))-\frac{k\log{k}}{\Delta\log{q}}}$ solves $\vkSUM(n,m,k,q)$ with advantage atmost $o(1)$.    
% \end{conjecture}



\subsection{Background about Lattices}
\label{sec:latback}

\shweta{Define discrete Gaussians and add the lemmas we need.}

 \begin{lemma}
 \label{lem:dgsizebd}
 \shweta{Bound the size of DG sample}
 \end{lemma}

%  \begin{definition}(Hard-to-invert function)\label{hardToInvert}\cite{tcc-2010-18746}
% Let $n$ be the security parameter and $\kappa = \omega(\log{n})$. A polytime computable function $\sf{f}:\{0,1\}^{n} \xrightarrow{} \Z_{q}^{*}$ is $2^{-\kappa}$ hard to-invert if for every PPT adversary $\mathcal{A}$
% \begin{align*}
%     \Pr_{\vecx \sample \mathcal{D}}[\mathcal{A}(\sf{f}(\vecx)) = \vecx] \leq 2^{-\kappa}
% \end{align*}
% where $\mathcal{D}$ is any polytime-sampleable distribution.
% \end{definition}
% \begin{definition}[Leaky sources]\label{leaky-sources}\cite{tcc-2010-18746}
%     let $\vecx$ be any random variable over $\{0,1\}^{n}$ and let $\sf{f}:\{0,1\}^{n} \xrightarrow{} \Z_{q}^{*}$ be any polytime computable function. $(\vecx,\sf{f}(\vecx))$ is called an $(n,\kappa)$ leaky source if it satisfies:
%     \begin{itemize}
%         \item {\textbf{Hard-to-invert leaky sources}}. $\vecx \sample \mathcal{D}$ where $\mathcal{D}$ is any polytime sampleable distribution and $\sf{f}$ is $2^{-\kappa}$- hard-to-invert.
%     \end{itemize}
% \end{definition}
\begin{lemma}(Leftover hash lemma)\label{lhl}(Section 2.2 of \cite{goldwasser2010robustness})
Let $(X,Z) \in \mathcal{X} \times \mathcal{Z}$ be any joint random variable over $\Z_{q}^{n}$ with min-entropy $H_{\infty}(X|Z) \geq k$. For any $\epsilon > 0$ and $m \leq \frac{k-2\log(\frac{1}{\epsilon})-O(1)}{\log{q}}$, the joint distribution of ($Z,\matC,\matC \cdot \vecs$) where $\matC \sampleU \Z_{q}^{m \times n}$ is uniformly random and $s \in \mathcal{X}$ is $\epsilon$-close to the uniform distribution over $(Z,\Z_{q}^{m \times n} \times \Z_{q}^{m})$. 
\end{lemma}
% \begin{lemma}(Goldreich-Levin theorem)\label{goldreich-levin}(Section 4, theorem 1 of \cite{tcc-2010-18746})
% Let $q$ be prime, and let $H$ be any polynomial size subset of $\Z_{q}$. Let $h: H^{n} \xrightarrow{} {\Z_{q}}^{m}$ be any (possibly randomized) function that is $2^{-\kappa}$ hard to invert. Let $\matC \sampleU \Z_{q}^{m \times n}$ be uniformly random and $\vecs$ be drawn from distribution $\mathcal{D}$ over $H^{n}$. Then
% \begin{align*}
% (\sf{f}(\vecx), \matC,\matC\vecs)\approx_{c}(\sf{f}(\vecx),\matC, \vecv)    
% \end{align*}
% where $\vecv \sampleU \Z_{q}^{m} $
% \end{lemma}
%\nikolaj{What does it mean to invert a randomized function?}\akhil{Let's take hardness of avg-case SIS problem  where $n\geq m\log{q}$(short vector here is anything $\leq \sqrt{n}$) the function be $\sf{f}(\vecx \in \{0,1\}^{n}) \triangleq \matA \vecx$ where $\matA \in \Z_{q}^{m\times n}$ is picked uniformly everytime, now the output of this function be $(\matA,\matA\vecx) \in \Z_{q}^{m \times n+1}$, it's hard to invert on $\vecx \in \{0,1\}^{n}$, I hope this makes sense. this is what I interpreted the above line to be.}
% Next we define the extended LWE problem \cite{ONPW11}.
% % \cite{cryptoeprint:2017/978}}
% \begin{definition}[Extended LWE]A PPT algorithm $\mathcal{A} = (\mathcal{A}_{1}, \mathcal{A}_{2})$ breaks
% extended $\lwe$ for noise distribution $\chi$ , $m$ samples, modulus $p$ and dimension $n$ if
% \begin{align*}
%     \abs{\Pr[\mathcal{A}_{2}(\sf{st}, \matA, \matA\vecs+\vece, \vecx, \vecx^{T}\vece) = 1]- \Pr[\mathcal{A}_{2}(\sf{st}, \matA, \matB, \vecx, \vecx^{T}\vece)]} \geq \epsilon
% \end{align*}
% where $(\vecx,\sf{st}) \sample \mathcal{A}_{1}(1^{n})$ and the randomness is taken over $\matA \sampleU \Z_{p}^{m \times n}, \matB \sampleU \Z_{p}^{m}, \vecs \sampleU \Z_{p}^{n}, \vece \sample \chi^{m}$ and a non-negligible $\epsilon$.
% \end{definition}
% \begin{lemma}[\cite{AP12}, Section 3, Theorem 1]\label{extended-lwe-AP12} 
% For dimension $n$, prime modulus $q$, $m \geq n+\omega(\log{n})$ samples and noise distribution $\chi$, if there is an algorithm solving extended $\lwe$ with probability $\epsilon$, then there is an algorithm solving $\lwe$ with advantage $\frac{\epsilon}{2q-1}$ as long as $q$ is an upper bound on the norm of the hint $\vecx^{T}\vece$.    
% \end{lemma}
% \begin{theorem}[LWE with hard-to invert auxiliary input]\label{lwe-aux}
%     Let $n$ be the security parameter. Assume $\lwe(m,n,q,\chi)$ is hard, then for every $(n,\kappa)$ leaky source $(\vecx,\sf{f}(\vecx))$ where $\kappa =\omega(\log{n})$ we have 
%     \begin{align*}
%         (\sf{f}(\vecx), \matA \matV, \matA \matV\vecx+\vece) \approx_{c} (\sf{f}(x),\matA \matV,\vecv)
%     \end{align*}
%     where $\matA \sampleU \Z_{q}^{n \times m}, \matV \sampleU \Z_{q}^{m \times n}, \vecv \sampleU \Z_{q}^{n}, \vece \sample \chi^{n}$
% \end{theorem}
% \begin{proof}
%     By Lemma \ref{goldreich-levin},
%     \begin{align*}
%         (\sf{f}(\vecx), \matV, \matV \vecx) \approx_{c} (\sf{f}(x),\matV,\vecy)
%     \end{align*}
%     where $\vecy \sampleU \Z_{q}^{m}$
%     \begin{align*}
%         \implies (\sf{f}(\vecx), \matA, \matV, \matA \matV \vecx + \vece) \approx_{c} (\sf{f}(x),\matA,\matV,\matA\vecy+\vece)
%     \end{align*}
%     By hardness of $\lwe(m,n,q,\chi)$, 
%     \begin{align*}
%     (\sf{f}(x),\matA,\matV,\matA\vecy+\vece) \approx_{c}  (\sf{f}(x),\matA,\matV,\vecv)
%     \end{align*}
% \end{proof}
\subsection{Public Key Encryption from $\kSUM$ and $\lwe$}


\subsubsection{Construction}
We describe our public key encryption scheme $\pke = (\setup, \enc, \dec)$ for message space $\cM=\{0,1\}$ below: 
\begin{description}
    \item $\pke.\setup(1^\secp)$: Upon input the unary representation of the security parameter $\secp$, do the following:
    \begin{enumerate}
    %\item Set $\Delta = \frac{1}{(\log{n})^{c}}\text{ ($c$ is any constant)}, k = \log{\log{n}}, q= 2^{\frac{k}{\Delta\log{\log{k}}}}, m =\frac{k \log{n}}{\Delta \log{q}}, \alpha = \frac{1}{4k}=\tilde{O}(1),\chi = \cD_{\Z_{q},\alpha q}$. %\shweta{The parameters all need to be stated as a function of $\secp$ or $n$.}
        \item Sample $\matA \sampleU \Z_{q}^{m \times n}$.
        \item Sample a set of indices $S \subseteq [n]$ uniformly such that  $\abs{S} = k$.
        \item Let $i$ be the smallest index in $S$. Let the $i^{th}$ column value i.e, $\veca_{i}$ in the matrix $\matA$ be replaced by $-\sum_{j \neq i \in S}\veca_{j}$.
        \item Let $\vecu \in \{0,1\}^{n}$ where $\vecu[j] = 1 \iff j \in S$.
        \item Output  $\pk := \matA$, $\sk := \vecu$.
    \end{enumerate}
    \item $\pke.\enc(\pk := \matA, \mu \in \{0,1\})$: Upon input the public key $\pk$ and the message $\mu$, do the following:
    \begin{enumerate}
        \item Sample $\vecs \sampleU \Z_{q}^{m}$.
        \item Compute $\vecc:= \vecs^{T}\matA+\vece^{T}+\floor{\frac{q}{2k}}\vecmu^{T}$ where $\vece \sample \chi^{n}$ and $\vecmu^{T} := [\mu~.~.~\mu]$ ($1\times n$ row vector).
%        \shweta{By default we are using column vectors and transposing to get rows. Let's be consistent.}\akhil{done!}
        \item Output $\ct := \vecc$.
    \end{enumerate}
      \item $\pke.\dec(\pk:= \matA, \sk := S, \ct := \vecc)$: Upon input the public key $\pk$, the secret key $\sk$ and the ciphertext $\ct$, do the following:
    \begin{enumerate}
    \item Let $c':=\vecc^{T}\vecu$. % \shweta{It is better to write $c'$ as an inner product of the ciphertext with a k sparse vector. Indeed, the k sparse vector should be the secret key.} \akhil{done! I retained step 1 and 2 of the PKE.setup because of how we defined kSUM}     
    \item If $\norm{c'}_{2} < \frac{q}{4}$ then output $0$ else output $1$.
    \end{enumerate}
\end{description}

We now prove the scheme satisfies correctness and CPA security.
\begin{theorem}[Correctness.]\label{pke:correctness}
    Let the parameters be chosen as described in Section \ref{sec:pke-params}. Then, the public key encryption scheme $\pke$ is weakly correct (Definition \ref{def:pke}).
\end{theorem}
\begin{proof}
\begin{align*}
    c' &= \vecc^{T}\vecu
    \\&=\vecs^{T}\matA\vecu + \vece^{T}\vecu+\floor{\frac{q}{2}}\mu
    \\&=0+\sum_{\vecu[j] = 1 } e_{j} + \floor{\frac{q}{2}}\mu
\end{align*}
Since by our choice of parameters (Section \ref{sec:pke-params}), we have that  $\sum_{\vecu[j] = 1} e_{j} < \frac{q}{4}$, correctness holds.
% Hence, when $\mu = 0$, the value  is $\sum_{j \in S} e_{i}^{T}$, if we show that $\sum_{j \in S} e_{i}^{T}< \frac{q}{4}$ then that would be sufficient.
% \newline 
% \newline 

%Therefore, for the parameters mentioned in $\pke.\setup$, 
%\shweta{Are these parameters for the scheme that survived or the scheme that was removed? The caption points to the scheme that was removed. Then, the dependence between the parameters should be explicitly described so that the choices become clear. Then the tradeoffs between the choices should be discussed. }\akhil{I have mentioned all the parameters explicitly in the setup and the trade-off in theorem 6.3}
% \newline
% \newline 
% It is worth noting that the previously best known $\pke$ scheme use $\alpha = \frac{1}{\tilde{O}(\sqrt{m})}$(section 5.2.1 of \cite{cryptoeprint:2015/939}). \shweta{Again, this needs to be stated in terms of $\secp$ because in typical LWE schemes $m = n \log q$ whereas for us $m$ is (much) smaller than $n$. So comparing in terms of $m$ is misleading.}
\end{proof}
\noindent
Next, we prove the security of our scheme under the hardness of LWE and $k$-SUM. We do this by first showing a reduction from $k$-SUM to vector-$k$-SUM in Lemma \ref{reduction-vkSUM} and then showing IND-CPA security relying on vector-$k$-SUM in Conjecture \ref{conj:vkSUM}.
%we proceed to show generic hybrid arguments based on the hardness of the above mentioned problems. Then, in Lemma. \ref{pke-security-tradeoff}, we argue why any PPT adversary won't be able to break the security of $\pke$ scheme.

\begin{theorem}[Security.]\label{security:pke}
    Assuming the hardness of $\vkSUM(n,m,k,q), \lwe(m,n,q,\chi)$ where the parameters are chosen as described in Section \ref{sec:pke-params}, the public key encryption scheme $\pke$ satisfies weak $\indcpa$ security (Definition \ref{def:pke}). %\shweta{I would like the theorem statement to be complete -- state parameters in terms of secp, quantify hardness of the two problems. For instance, I believe we are using subexp hardness of LWE? This is not evident here.}
\end{theorem}
\begin{proof}
We prove the theorem via a sequence of hybrids between the challenger and a PPT adversary $\cA$.
\begin{description}
    \item {\sf Hybrid 0}: This is the real world with challenge bit $0$. This is same as $\pkeGame^{0}_{\cA(n)}$
    \item {\sf Hybrid 1}: This world is same as {\sf Hybrid 0} except we sample public key $\pk$ as $\matA' \sampleU \Z_{q}^{m\times n}$.
    \item {\sf Hybrid 2}: This world is same as {\sf Hybrid 1} except we replace the cipher-text $\ct :=\vecs^{T}\matA'+\vece^{T}+\floor{\frac{q}{2k}}\vecmu_{0}^{T}$ by $\vecv^{T}$ where $\vecv \sampleU \Z_{q}^{n}$.
\end{description}
In {\sf Hybrid 2}, the distribution seen by the adversary is independent of the challenge bit $b$ hence the advantage of the adversary in this world is negligible.

\paragraph{Indistinguishability of Hybrids.} We now show that consecutive hybrids are indistinguishable.
%\shweta{Expand this.}\akhil{done! Please let me know if any changes must be done}
\begin{claim}
   Assume that $\vkSUM(n,k,q,\Delta)$ is hard (Conjecture \ref{conj:vkSUM}) for the parameters described in Section \ref{sec:pke-params}. Then, {\sf Hybrid 0} and {\sf Hybrid 1} are indistinguishable.
\end{claim}
\begin{proof}
Let $\cD$ be a PPT adversary that distinguishes {\sf{Hybrid} 0} from {\sf{Hybrid} 1} with advantage $\epsilon$. Let $\cC$ be the $\vkSUM(n,m,k,q)$ challenger. Then we give a reduction $\cB$ that solves $\vkSUM(n,m,k,q)$ with advantage $\epsilon$ as follows:
\begin{enumerate}
    \item $\cC$ outputs $\matA^{*}$.
    \item $\cB$ samples $\mu_{0},\mu_{1} \sample \cM, \vecs \sampleU \Z_{q}^{m}$, $\vece \sample \chi^{n}$
    \item $\cB$ then computes $(\mu_{0},\mu_{1},\matA^{*},\vecs^{T}\matA^{*}+\vece^{T}+\floor{\frac{q}{2k}}\vecmu_{0}^{T})$ and runs $\cD$ on this.
    \item If $\cD$ outputs $b$ then $\cB$ outputs b
\end{enumerate}
Notice that when $\cC$ outputs $\matA' \sampleU \Z_{q}^{m \times n}$ then $\cB$ simulates {\sf Hybrid 0} else, it simulates {\sf Hybrid 1}. Hence, $\cB$ solves $\vkSUM(n,m,k,q)$ with probability equal to the advantage of $\cD$ i.e, $\epsilon$.
\newline 
\newline 
From conjecture \ref{conj:vkSUM}, any PPT adversary can distinguish the above hybrids with atmost $\epsilon = o(1)$ probability.
Therefore, by the hardness of $\vkSUM(n,m,k,q)$, we have
    \begin{align*}
 (m_{0},m_{1},\matA,\vecs^{T}\matA+\vece^{T}+\floor{\frac{q}{2k}}\vecmu_{0}^{T}) \approx_{c}  (m_{0},m_{1},\matA',\vecs^{T}\matA'+\vece^{T}+\floor{\frac{q}{2k}}\vecmu_{0}^{T})
\end{align*}
\end{proof}
% As part of $\pkeGame_{\cA(\secp)}^{0}$ the view of the PPT adversary $\cA$ is $(m_{0},m_{1},\matA,\vecs^{T}\matA+\vece^{T}+\floor{\frac{q}{2k}}\vecm_{0})$ where all the elements in this distribution are sampled as in $\pkeGame^{0}_{\cA(\secp)}$.
% \begin{align*}
%  (m_{0},m_{1},\matA,\vecs^{T}\matA+\vece^{T}+\floor{\frac{q}{2k}}\vecm_{0}) \approx_{c}  (m_{0},m_{1},\matA',\vecs^{T}\matA'+\vece^{T}+\floor{\frac{q}{2k}}\vecm_{0})
% \end{align*}
% where $\matA' \sampleU \Z_{q}^{m\times n}$. The above relation holds due to the hardness of $\vkSUM(n,k,q,\Delta)$.
\begin{claim}
     Assume that $\lwe(m,n,q,\chi)$ is hard (Theorem \ref{lwe-hardness-param}) for the parameters described in Section \ref{sec:pke-params}. Then, {\sf Hybrid 1} and {\sf Hybrid 2} are indistinguishable.
\end{claim}
\begin{proof}
Let $\cD$ be a PPT adversary that distinguishes {\sf{Hybrid} 1} from {\sf{Hybrid} 2} with advantage $\epsilon$. Let $\cC$ be the $\lwe(m,n,q,\chi)$ challenger. Then we give a reduction $\cB$ that solves $\lwe(m,n,q,\chi)$ with advantage $\epsilon$ as follows:
\begin{enumerate}
    \item $\cC$ outputs the $\lwe(m,n,q,\chi)$ challenge $(\matA',\vecy)$.
    \item $\cB$ samples $\mu_{0},\mu_{1} \sample \cM$
    \item $\cB$ then computes $(\mu_{0},\mu_{1},\matA',\vecy+\floor{\frac{q}{2k}}\vecmu_{0}^{T})$ and runs $\cD$ on this.
    \item If $\cD$ outputs $b$ then $\cB$ outputs b
\end{enumerate}
Notice that when $\cC$ outputs $\vecy = \vecs^{T}\matA'+\vece^{T}$ then $\cB$ simulates {\sf Hybrid 1} else, it simulates {\sf Hybrid 2}. Hence, $\cB$ solves $\lwe(m,n,q,\chi)$ with advantage equal to the advantage of $\cD$ i.e, $\epsilon$.
\newline 
\newline 
By the hardness of $\lwe(m,n,q,\chi)$ where $\chi$ is parameterised by $\alpha q$, $\epsilon = \negl(\secp)$. Hence, we have that
\begin{align*}(m_{0},m_{1},\matA',\vecs^{T}\matA'+\vece^{T}+\floor{\frac{q}{2k}}\vecmu_{0}^{T}) \approx_{c} (m_{0},m_{1},\matA',\vecv^{T})
\end{align*}
where $\matA' \sampleU \Z_{q}^{m \times n}$, $\vecv \sampleU \Z_{q}^{n}$. 
\end{proof}
% \begin{align*}
% &(m_{0},m_{1},\matA',\vecs^{T}\matA'+\vece^{T}+\floor{\frac{q}{2k}}\vecm_{0}) \approx_{c} (m_{0},m_{1},\matA',\vecu^{T})
% \end{align*}
% where $\matA' \sampleU \Z_{q}^{m \times n}$, $\vecu \sampleU \Z_{q}^{n}$. The above relation holds due to the hardness of $\lwe(m,n,q,\chi)$ where $\chi$ is parameterised by $\alpha q$.
% \begin{align*}
% (m_{0},m_{1},\matA',\vecu^{T}) \approx_{s} (m_{0},m_{1},\matA',\vecu^{T}+\floor{\frac{q}{2k}}\vecm_{1})
% \end{align*}
% where $\matA' \sampleU \Z_{q}^{m \times n}$, $\vecu \sampleU \Z_{q}^{n}$. This is because of adding $m_{1}$ to a uniformly random value. Now, on again unwrapping the above equation in a similar way would result in 

% \begin{align*}
%  (m_{0},m_{1},\matA',\vecu^{T}+\floor{\frac{q}{2k}}\vecm_{1}) \approx_{c}(m_{0},m_{1},\matA,\vecs^{T}\matA+\vece^{T}+\floor{\frac{q}{2k}}\vecm_{1})
% \end{align*}
% where all the elements in this distribution are sampled as in $\pkeGame^{1}_{\cA(\secp)}$ on the rhs. 
Therefore, for any PPT adversary $\cA$: 
        \begin{equation*}     \big|\Pr[\pkeGame_{\cA(\secp)}^{0} = 1] - \Pr[\pkeGame_{\cA(\secp)}^{1} = 1]\big| \leq  o(\secp)
        \end{equation*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Parameters}
\label{sec:pke-params}
Here, we enumerate the constraints that need to be satisfied for correctness and security to hold, and provide an instantiation.
\begin{enumerate}
    \item For correctness to hold, from Theorem \ref{pke:correctness} we need  $\sum_{j \in S} e_{j}< \frac{q}{4}$. Note that $\sum_{j \in S} e_{j} \leq k (\alpha q)$ with high probability \ref{lem:dgsizebd}. Therefore, for the correctness to hold, we need $k\alpha q \leq \frac{q}{4}$ which implies $\alpha \leq \frac{1}{4k}$.
 \item For security, we need that minimum time taken by an adversary to solve $\vkSUM(n,k,q,\Delta)$ is super-polynomial in $n$. Thus, from Lemma \ref{conj:vkSUM}, we require that $n^{\frac{k}{2}-\frac{k \log{k}}{\Delta \log{q}}} = n^{\omega(1)}$. 
        \item Additionally, we require that the minimum time taken by an adversary to solve $\lwe(m,n,q,\chi = \tilde{O}(1))$ is super-polynomial in $n$. From Section \ref{def:assumptions}, this implies that $2^{\tilde{O}(\frac{{m}}{1.5\log{m}})}$ must be $n^{\omega(1)}$. 
        \item From Theorem \ref{lwe-hardness-param}, we require $q\geq 2\sqrt{m}k$.
%$\alpha = \frac{1}{4(\log{\log{n}})}$ works which is $\alpha = \tilde{O}(1)$.
\end{enumerate}


% \begin{lemma}\label{pke-security-tradeoff}
%     For the cryptosystem mentioned in this section ($\pke$) to be secure against a PPT adversary, we need to ensure that :
%     \begin{enumerate}
%         \item $n^{\frac{k}{2}-\frac{k \log{k}}{\Delta \log{q}}}$ is super-polynomial in $n$. (This is the minimum time taken by an adversary to solve $\vkSUM(n,k,q,\Delta)$ from Lemma \ref{reduction-vkSUM} and Conjecture.\ref{conj:KSUM})
%         \item $2^{\tilde{O}(\frac{{m}}{1.5\log{m}})}$  is super-polynomial in $n$ (This is the minimum time taken by an adversary to solve $\lwe(m,n,q,\chi = \theta(1))$).refer to Section.\ref{def:assumptions} and Shweta's comments above.)  
%         \item $q\geq 2\sqrt{m}k$ (From theorem.\ref{lwe-hardness-param}).
%     \end{enumerate}
% \end{lemma}
To satisfy these constraints, we set parameters as follows:
\begin{align*}
    &\Delta = \frac{1}{\log{n}},   & k &= (\log{\log{n}})^{c} = \omega(1),  &q &= n^{(\log{\log{n}})^{c''}} = n^{\omega(1)},\\
    & m = (\log{n})(\log{\log{n}})^{c''}, &\alpha &= \frac{1}{4k} = \frac{1}{(\log{\log{n}})^{c}} = \tilde{O}(1) & \mbox{}{}
\end{align*}
where $c,c',c''$ are any constants such that $c = c'+c''$ and $c\geq 2, c'' \geq 1$. 


\paragraph{Hardness for our choice of parameters.}
Next, we discuss the hardness of the underlying problems for our choice of parameters:
\begin{enumerate}
    \item {\bf k-SUM:} From the above parameters and Conjecture \ref{conj:vkSUM}, the $\vkSUM(n,m,k,q)$ when instantiated with $k = (\log{\log{n}})^{c}$, $q = n^{(\log{\log{n}})^{c''}} = n^{\omega(1)}$, $m = (\log{n})(\log{\log{n}})^{c''}$, cannot be solved by any PPT adversary with probability greater than $o(1)$, because the minimum time required would be $n^{\omega(1)}$. This, by the reduction given in Lemma \ref{reduction-vkSUM} implies that $\kSUM(n,k,q)$ when instantiated with the above parameters cannot be solved by any PPT adversary with probability greater than $o(1)$.
    \item {\bf LWE:} From the above parameters and Lemma \ref{lwe-hardness-param}, $\lwe(m,n,q)$ instantiated with $m = (\log{n})(\log{\log{n}})^{c''}$ $N=n,q=n^{(\log{\log{n}})^{c''}}$ cannot be solved with greater than $\negl(\secp)$ by any adversary running in less than $n^{\omega(1)}$. \shweta{Discuss that the worst-case to average-case reduction still works for our regime of parameters.}
\end{enumerate}

\paragraph{Tradeoffs between Parameters.}
As can perhaps be expected, the hardness of each of our two assumptions can be traded against the other. First, we note that the $k$-SUM problem becomes easy to solve at lower densities and that a greater value of $\alpha$ in $\lwe$ translates to a weaker (i.e. better) $\lwe$ assumption. Focusing on $\Delta = \frac{k \log{n}}{m\log{q}}$, and $\alpha \leq \frac{1}{4k}$ helps us see that as $k$ decreases, the noise rate of $\lwe$ i.e, $\alpha$ increases. On the other hand, increase in $\alpha$ results in decreased $\Delta$, leading to a trade-off between how large $\alpha$ can be versus how small $\Delta$ can be. Similarly, as the dimension of the $\lwe$ secret $m$ increases, we see that $\Delta$ decreases. Thus, to avoid making overly aggressive assumptions on $\kSUM$ (which is comparatively less studied) forces us to assume exponential hardness of $\lwe$ (which is much better understood). Fixing $\Delta,q$ and increasing $m$ comes at the cost of increasing the value of $k$, which in turn decreases $\alpha$, resulting in a worse $\lwe$ assumption. 

Our focus is on the parameter $\alpha$ and $\Delta$ because those are the ones affecting $\lwe$ and $\vkSUM$ hardness significantly. Hence, we take the minimum value that $m$ can take and then perform the trade-off between $\alpha$ and $\Delta$.\medskip
% \shweta{Discuss the quality of LWE noise rate and k-SUM density, and the tradeoff between these. If I recall correctly, we wanted the dimension of the lwe secret to be small (thus needing subexp security) due to k-SUM -- if the dimension of the secret is too large, the density at which we need to assume the security of k-SUM is too small (due to m being in the denominator?). Editorial: the parameters used in the definition of LWE, and indeed in all our problems, are inconsistent. }\akhil{Believe that this needs improvement, but would like some feedback before changing any further}. 

We would also want $q \geq n^{c}$ where $c \in \{\text{constant}, \omega(1)\}$ because very small $q$ results in trivially solving the underlying lattice problem. But, for our requirements (especially, (3) and $\alpha = \tilde{O}(1)$), for any of the above $q$, $\Delta \leq  \tilde{O}(\frac{1}{\log{n}})$. Therefore, while the parameters of our construction can be improved (for ex, we can take: $k = (\log{m})^{c}$ where $c$ is some constant), the two important parameters $\alpha$ and $\Delta$ won't be significantly improved. However, we like to point out that $\Delta$ value can be made closer to constant by reducing $q$ to a value of the order $n^{\frac{1}{\omega(1)}}$.

\begin{comment}
\subsection{PKE from ``just our'' LWE.}
It is important to understand whether exponential hardness of LWE with super-constant modulus to noise ratio qualifies as a ``minicrypt'' assumption. Here, we argue that it does. 

Let us compare with the version of PKE that LWE twice (without using LHL). The public key is a random matrix and its LWE sample. During encryption, you treat the LWE in the PK as random, and use LWE again, this time with a small secret, multiplied on the other side. Decryption is obvious. You lose a bit in parameters when you use a small secret -- I don't recall how much. We can use the same LWE as we use in our construction for the PK. I expect the noise in the CT LWE sample will be larger by factor $n$. 
\end{comment}

% \begin{itemize}
%     \item Point 1 implies that $\frac{k}{2}-\frac{k \log{k}}{\Delta \log{q}} \text{ must be } \omega(1)$. For our choice of parameters, this becomes $\frac{k}{2}-\log{\log{k}} \log{k}$. Hence, this condition is satisfied. 
%     \item In Point 2, let's ignore the $\log{m}$ factor because of $\tilde{O}$ then very roughly this translates to $2^{m} = 2^{\frac{k\log{n}}{\Delta\log{q}}}$ (By the definition of $\Delta$) (\akhil{We need to be much more stricter with this, but for time being}) which translates to $n^{\frac{k}{\Delta\log{q}}}$. Therefore, to satisfy this condition $\frac{k}{\Delta\log{q}}$ must be $\omega(1)$. By our parameters the value of $\frac{k}{\Delta \log{q}} = \log{\log{k}}\approx\log{\log{\log{n}}}$ and hence this condition is also satisfied.
%     \item From our parameters, notice that $q = 2^{\frac{k}{\Delta \log{\log{k}}}} \implies q = n^{\frac{c \log{\log{n}}}{\log{\log{k}}}}$ which is greater than $2\sqrt{\log{n}}$ and hence the third condition also holds.
%     \akhil{This is wrt the bounds of  search version of vkSUM, we need to be wary of the constraints for a decision version}
% \end{itemize}



% \begin{corollary}
%     There exists no polynomial-time algorithm to solve $\vkSUM(n,k,q,\Delta)$ if we assume the hardness of $\kSUM(n,k,\Delta)$ at $k=\omega(1)$ whenever $q \geq 2^{\frac{k}{\Delta \log{\log{k}}}}$.\shweta{reword}
% \end{corollary}
% \begin{proof}
%     Observe that $\frac{k\log{k}}{\Delta\log{q}}$ is $o(k)$ whenever \shweta{This trailed off. Please complete.}
% \end{proof}

\begin{comment}
\subsubsection{Version 2 (non-vector $k$-SUM)}\label{pkeV2}
Our public key encryption scheme $\pke = (\setup, \enc, \dec)$ for message space $\cM=\{0,1\}$, is described as follows: 
\begin{description}
    \item $\pke.\setup(1^\secp)$: Upon input the unary representation of the security parameter $\secp$, do the following:
    \begin{enumerate}
    \item  Parameters $n=\secp, \Delta = \Delta(\secp), k =k(\secp), m=\frac{k \log{n}}{\Delta \log{q}}, \chi = \chi(\secp):=\cD_{\Z_{q},\alpha q}$ (i.e, each element in $\chi$ is bounded by the value $\alpha q$ with high probability) and let $q = 2\sqrt{k\cdot \log{n} \cdot \omega(1)}+2$. 
        \item $\matA \sampleU (\Z_{q}^{m})^{n}$
        \item Sample $\vece \in \{0,1\}^{n}$ uniformly such that  $\norm{\vece}_{0} = k$
        \item Let $\vecu := \matA \odot \vece$
        \item Output  $\pk := (\vecu,\matA)$, $\sk := \vece$
    \end{enumerate}
    \item $\pke.\enc(\pk := (\vecu,\matA), \mu \in \{0,1\})$: Upon input the public key $\pk$ and the message $m$, do the following:
    \begin{enumerate}
        \item Compute $\vecp := \matA^{T}\vecs + \vecv $ where $\vecs \sample \chi^{m},\vecv \sample \chi^{n}$
        \item Compute $c:= \vecu^{T}\vecs+\vecv'+\floor{\frac{q}{2}}\mu$ where $\vecv' \sample \chi$
        \item Output $\ct := (\vecp,c)$
    \end{enumerate}
      \item $\pke.\dec(\pk:= (\vecu, \matA), \sk := \vece, \ct := (\vecp,c))$: Upon input the public key $\pk$, the secret key $\sk$ and the ciphertext $\ct$, do the following:
    \begin{enumerate}
        \item Compute $\mu' := c-\vece^{T}\vecp$.
        \item If $\norm{\mu'}_{2} < \frac{q}{4}$ then output $0$ else output $1$.
    \end{enumerate}
\end{description}
We now prove the scheme satisfies correctness and CPA security.
\begin{lemma}[Hoeffding Bound]\label{hoeffding-bound}
Let $X_{1},~.,~.,~X_{n}$ be independent random variables in the range $[a,b]$ and let $X =\sum_{i=1}^{n} X_{i}$. Then,
\begin{equation*}
    \Pr[\abs{X-\exp{X}} \geq t] \leq 2e^{\frac{-2t^{2}}{n(a-b)^{2}}}
\end{equation*}
\end{lemma}
\begin{theorem}[Correctness.]
      For any $\secp$, let parameters of the $\pke$ construction be set as in table \ref{paramTablePKEV2}. Then, the public key encryption scheme $\pke$ described above is correct.
\end{theorem}
\begin{proof}
Note that for any $\matA \in (\Z_{q}^{m})^{n}$, $\vece \in \{0,1\}^{n}$, $\matA \odot e$ can be thought of as $\matA \vece + \vecc$ where $\vecc$ is the carry vector imagining we do simple addition in base-$q$. 
% \begin{comment}
%add this only if extra expostion is required to explain the idea behind carry
\newline 
\newline 
Computing $\matA \odot \vece$ can be basically done as follows:
\begin{itemize}
    \item $c_{1} = 0$
    \item for $i = 1$ to $m$:
    \begin{itemize}
        \item $b_{i} = c_{i}+\tilde{\veca}_{i}\vece \mod{q}$ where $\tilde{\veca}_{i}$ is the $i$-th row of $\matA$.
        \item $c_{i+1} = \nearest{\frac{c_{i}+\tilde{\veca_{i}}\vece}{q}} \mod{q}$.
\end{itemize}
\item Output $\vecb^{T} = [ b_{1}~.~.~b_{m}]$
\end{itemize}
% \end{comment}
% \newline 
% \newline 
Notice that each carry element depends on previous carry element and current row summation according to $e$. To facilitate a better analysis of bounds, we would like to divide a carry vector element $c_{i}$ into an independent part ($x_{i}$) and a dependent part ($y_{i}$) that depends on $c_{i-1}$.
\newline 
\newline 
Computing $\matA \odot \vece$ can be done as follows:
\begin{itemize}
    \item $x_{1} = 0, y_{1} = 0$
    \item for $i = 1$ to $m$:
    \begin{itemize}
        \item $b_{i} = x_{i}+y_{i}+\tilde{\veca}_{i}\vece \mod{q}$ where $\tilde{\veca}_{i}$ is the $i$-th row of $\matA$.
        \item $x_{i+1} = \floor{\frac{\tilde{\veca_{i}}\vece}{q}} \mod{q}$.
        \item $y_{i+1} = \floor{\frac{x_{i}+y_{i}+\tilde{\veca_{i}}\vece}{q}}-x_{i+1} \mod{q}$.
\end{itemize}
\item Output $\vecb^{T} = [ b_{1}~.~.~b_{m}]$
\end{itemize}
\begin{claim}\label{x-bound}
From the algorithm to compute $\matA \odot \vece$ where $\vecc = \vecx+\vecy$. 
    For any fixed $\vece \in \{0,1\}^{n} \ni \norm{\vece}_{0} = k$, 
    \begin{align*}
    \forall i \in [m],~\Pr_{\matA \sampleU (\Z_{q}^{m})^{n}}[\abs{x_{i}} \geq \sqrt{ k \cdot \log{n}\cdot \omega(1)}] \leq 2e^{-2\log{n}\cdot \omega(1)}
    \end{align*}
\end{claim}
From the algorithm to compute $\matA \odot \vece$, $\vecc = \vecx+\vecy$. For a fixed $\vece \in \{0,1\}^{n} \ni \norm{\vece}_{0} = k$, after fixing $\vece$, we can denote value of each $\tilde{\veca_{i} \vece}$ as a summation of $k$ independent values that take values from $[\frac{-(q-1)}{2},\frac{q-1}{2}]$ and as $\matA$ is picked uniformly, $\exp{\tilde{\veca_{i} \vece}}= 0$. Therefore for any $i \in [m]$, by Hoeffding bound (\ref{hoeffding-bound}) 
    \begin{align*}
    ~\Pr_{\matA \sampleU (\Z_{q}^{m})^{n}}[\abs{\tilde{\veca_{i}}\vece} \geq q\sqrt{ k \cdot \log{n}\cdot \omega(1)}] \leq 2e^{-2\log{n}\cdot \omega(1)}
    \end{align*}
    Therefore, for any $i \in [m]$, with probability $1-n^{-\omega(1)}$,  $\abs{x_{i}} \leq \sqrt{k\cdot \log{n} \cdot \omega(1)} \leq \frac{q-1}{2}$ and notice that $\exp{x_{i}} = 0$ over randomness of sampling ${\matA \sampleU (\Z_{1}^{m})^{n}}$.
    \begin{claim}\label{y-bound}
    $\forall~i \in [m], \abs{y_{i}} \leq 1$ with probability $1-n^{\omega(1)}$.
    \end{claim}
    \begin{proof}
        Notice that $\abs{y_{0}} \leq 1 $, then assuming that it is true for $y_{i}$ we will show by induction that it is true for all the values.
        \begin{align*}
            \abs{y_{i+1}} &= \abs{\floor{\frac{x_{i}+y_{i}+\tilde{\veca_{i}}\vece}{q}}-x_{i+1} \mod{q}}
            \\&\leq \abs{\floor{\frac{x_{i}+y_{i}}{q}}+1}
            \\&\leq 1. (\because \text{ $\abs{x_{i}} \leq \sqrt{k\cdot \log{n} \cdot \omega(1)} \leq \frac{q-1}{2}$ with $1-n^{\omega(1)}$ probability})
        \end{align*}
    \end{proof}
Now, coming back to the proof of correctness, 
\begin{align*}
    \mu' &= c-\vece^{T}\vecp
    \\&= \vecu^{T}\vecs+v'+\floor{\frac{q}{2}}\mu-\vece^{T}\matA^{T}\vecs-\vece^{T}\vecv.
    \\&= (\matA \odot e)^{T}\vecs+v'+\floor{\frac{q}{2}}\mu-\vece^{T}\matA^{T}\vecs-\vece^{T}\vecv.
    \\&= (\matA \vece +\vecc)^{T}\vecs+v'+\floor{\frac{q}{2}}\mu-\vece^{T}\matA^{T}\vecs-\vece^{T}\vecv.
    \\&= \bcancel{\vece^{T} \matA^{T} \vecs} +\vecc^{T}\vecs+v'+\floor{\frac{q}{2}}\mu-\bcancel{\vece^{T}\matA^{T}\vecs}-\vece^{T}\vecv.
\end{align*}
Hence, when $\mu = 0$, the value  is $v'-\vece^{T}\vecv+\vecc^{T}\vecs$, if we show that $\norm{v'-\vece^{T}\vecv+\vecc^{T}\vecs}_{2} < \frac{q}{4}$ then that would be sufficient.
\newline 
\newline 
From claim \ref{x-bound}, claim \ref{y-bound}, we can say that,\footnote{The bounds for $\vece^{T}\vecv,~\vecx^{T}\vecs$ are derived using hoeffding bound from lemma \ref{hoeffding-bound} similar to the bound on $x_{i}$ that we derived before}
\begin{align*}
    \norm{v'-\vece^{T}\vecv+\vecc^{T}\vecs}_{2} 
    &\leq \norm{v'-\vece^{T}\vecv+\vecx^{T}\vecs+\vecy^{T}\vecs}_{2}
    \\&\leq \beta+\sqrt{{k}\cdot \log{n}\cdot \omega(1)}\beta+\sqrt{m \cdot k\cdot \log{n} \cdot \omega(1)}\beta+\sqrt{m}\beta
\end{align*}
For convenience, we will merge terms of lower significance and use a constant $\sf{C}, \sf{C}'$ instead.
\begin{align*}
    \norm{v'-\vece^{T}\vecv+\vecc^{T}\vecs}_{2} &\leq \sf{C}(\sqrt{m\cdot k \cdot \log{n}\cdot \omega(1)}+m)\beta
    \\&\leq\sf{C'}(m\cdot\sqrt{\Delta \cdot \log{q}\cdot \omega(1)} +m)\beta (\because \Delta = \frac{k\log{n}}{m \log{q}}).
    \\&\leq \tilde{O}(m\cdot\sqrt{\Delta\cdot \omega(1)})\beta \text{ (ignoring $\log$ factors in $m$)}.
    \\&\leq\tilde{O}(m\cdot\sqrt{\Delta})\beta \text{ (assuming $\omega(1)$ is of the order $\log{\log{n}}$ and ignoring $\log$ factors in $m$)}.
\end{align*}
Now, if $\beta = \alpha q$ then $\alpha < \frac{1}{\tilde{O}(m\cdot\sqrt{\Delta\cdot \omega(1)})}$
\newline 
\newline 
Therefore, the correctness holds for the parameters as set in the table \ref{paramTablePKEV2}.
\newline
\begin{center}
\begin{tabularx}{0.8\textwidth} { 
  | >{\raggedright\arraybackslash}X 
  | >{\centering\arraybackslash}X 
  | >{\raggedleft\arraybackslash}X | }
 \hline
 $\Delta (= \frac{k\log{n}}{m\log{q}})$ & $k$ & $\alpha$ \\
\hline
 $1$  & $\omega(1)$  & $\frac{1}{\tilde{O}(m\sqrt{\omega(1)})}\footnote{\text{Here, we can use $\tilde{O}(m)$ assuming $\omega(1)$ is around $\log{\log{n}.}$ }}$\\
\hline
 $\frac{1}{\polylog(m)}$  & $\sf{\omega(1)}$  & $\frac{1}{\tilde{O}(m)}$\\
\hline
\end{tabularx}
\end{center}
\captionof{table}{Parameters of the PKE candidate in \ref{pkeV2}}\label{paramTablePKEV2}
It is worth noting that the previously best known $\pke$ scheme use $\alpha = \frac{1}{\tilde{O}(\sqrt{m})}$(section 5.2.1 of \cite{cryptoeprint:2015/939}).
\end{proof}
\begin{theorem}[Security.]
      For any $\secp \in \Z$, assume the parameters of $\pke$ scheme are as set in table \ref{paramTablePKEV2}, then assuming the hardness of $\kSUM(n,k,\Delta), \lwe(m,n,q,\chi)$, the public key encryption scheme $\pke$ described above satisfies $\indcpa$ security (Definition \ref{def:pke}).
    \begin{proof}
        The proof is exactly same as the one in theorem \ref{security:pke} but instead of using $\vkSUM(n,k,\Delta)$, we use $\kSUM(n,k,\Delta)$.
    \end{proof}
\end{theorem}
\end{comment}

